Optimizing Machine Learning Inference Queries with Correlative Proxy Models

We consider accelerating machine learning (ML) inference queries on unstructured datasets. Expensive operators such as feature extractors and classifiers are deployed as user-defined functions(UDFs), which are not penetrable with classic query optimization techniques such as predicate push-down. Recent optimization schemes (e.g., Probabilistic Predicates or PP) assume independence among the query predicates, build a proxy model for each predicate offline, and rewrite a new query by injecting these cheap proxy models in the front of the expensive ML UDFs. In such a manner, unlikely inputs that do not satisfy query predicates are filtered early to bypass the ML UDFs. We show that enforcing the independence assumption in this context may result in sub-optimal plans. In this paper, we propose CORE, a query optimizer that better exploits the predicate correlations and accelerates ML inference queries. Our solution builds the proxy models online for a new query and leverages a branch-and-bound search process to reduce the building costs. Results on three real-world text, image and video datasets show that CORE improves the query throughput by up to 63% compared to PP and up to 80% compared to running the queries as it is.

==> code/code.tex <==
 

==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/p1.java.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{p1} \PY{p}{(}\PY{k+kt}{int} \PY{n}{EMPNO}\PY{p}{,} \PY{n}{String} \PY{n}{ENAME}\PY{p}{,} \PY{k+kt}{int} \PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZob{}}
  \PY{k}{if} \PY{p}{(}\PY{n}{DEPTNO} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{k}{if}\PY{p}{(}\PY{n}{DEPTNO}\PY{o}{+}\PY{l+m+mi}{5}\PY{o}{\PYZgt{}} \PY{n}{EMPNO}\PY{p}{)}\PY{p}{\PYZob{}}
      \PY{k}{return} \PY{p}{(}\PY{n}{EMPNO}\PY{p}{,}\PY{n}{ENAME}\PY{p}{,}\PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}
\PY{n}{p2} \PY{p}{(}\PY{k+kt}{int} \PY{n}{EMPNO}\PY{p}{,} \PY{n}{String} \PY{n}{ENAME}\PY{p}{,} \PY{k+kt}{int} \PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZob{}}
  \PY{k}{if} \PY{p}{(}\PY{n}{DEPTNO} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{k}{if}\PY{p}{(}\PY{l+m+mi}{15}\PY{o}{\PYZgt{}} \PY{n}{EMPNO}\PY{p}{)}\PY{p}{\PYZob{}}
      \PY{k}{return} \PY{p}{(}\PY{n}{EMPNO}\PY{p}{,}\PY{n}{ENAME}\PY{p}{,}\PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/q1.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{TABLE} \PY{n}{EMP}\PY{p}{(}\PY{n}{EMPNO} \PY{n+nb}{int}\PY{p}{,} \PY{n}{ENAME} \PY{n}{String}\PY{p}{,} \PY{n}{DEPTNO} \PY{n+nb}{int}\PY{p}{)}\PY{p}{;}
\PY{n}{Case1}\PY{p}{:}
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
     \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t} 
    \PY{k}{WHERE} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{t}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
     \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t1} 
    \PY{k}{WHERE} \PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{t1}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{;} 

\PY{n}{Case2}\PY{p}{:}
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{AS} \PY{n}{EMP} 
        \PY{k}{WHERE} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO} \PY{o}{=} \PY{l+m+mi}{10} \PY{k}{AND} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO} \PY{k}{IS} \PY{k}{NOT} \PY{k}{NULL}\PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP0}\PY{p}{.}\PY{n}{EMPNO} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{AS} \PY{n}{EMP0} 
        \PY{k}{WHERE} \PY{n}{EMP0}\PY{p}{.}\PY{n}{EMPNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{;} 
\end{Verbatim}


==> code/q2.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{,} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DNAME} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{JOIN} \PY{n}{DEPT}
      \PY{k}{ON} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{=} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DEPTNO} \PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
      \PY{p}{(}\PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{,} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DNAME} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{LEFT} \PY{k}{OUTER} \PY{k}{JOIN} \PY{n}{DEPT}
         \PY{k}{ON} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{=} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{)}
    \PY{k}{WHERE} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DNAME} \PY{k}{IS} \PY{k}{NOT} \PY{k}{NULL}
\end{Verbatim}


==> code/q3.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{k}{COUNT}\PY{p}{(}\PY{o}{*}\PY{p}{)} \PY{k}{FROM}
      \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
        \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t} 
      \PY{k}{WHERE} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{t}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{)}\PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{k}{COUNT}\PY{p}{(}\PY{o}{*}\PY{p}{)} \PY{k}{FROM}
      \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
        \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t1} 
      \PY{k}{WHERE} \PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{t1}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{)}\PY{p}{;} 
\end{Verbatim}


==> code/q4.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
  \PY{k}{TABLE} \PY{n}{EMP}\PY{p}{(}\PY{n}{EMPNO} \PY{n+nb}{int}\PY{p}{,} \PY{n}{ENAME} \PY{n}{String}\PY{p}{,} \PY{n}{DEPTNO} \PY{n+nb}{int}\PY{p}{,}\PY{n}{SAL} \PY{n+nb}{int}\PY{p}{)}\PY{p}{;}
  \PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{,} \PY{k}{SUM}\PY{p}{(}\PY{n}{EMP}\PY{p}{.}\PY{n}{SAL}\PY{p}{)} 
      \PY{k}{FROM} \PY{n}{EMP} \PY{k}{GROUP} \PY{k}{BY} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}
  \PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{,} \PY{k}{SUM}\PY{p}{(}\PY{n}{t}\PY{p}{.}\PY{n}{sum1}\PY{p}{)} \PY{k}{FROM} \PY{p}{(}
   \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{,} \PY{k}{SUM}\PY{p}{(}\PY{n}{EMP}\PY{p}{.}\PY{n}{SAL}\PY{p}{)} \PY{k}{as} \PY{n}{sum1}
    \PY{k}{FROM} \PY{n}{EMP} \PY{k}{GROUP} \PY{k}{BY} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{)} \PY{k}{AS} \PY{n}{t} \PY{k}{GROUP} \PY{k}{BY} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO}
\end{Verbatim}


==> code/r1.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} 
\PY{n}{cond1}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{n}{v2} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{o}{!}\PY{n}{n2} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0}\PY{p}{)} \PY{p}{)} 
\PY{n}{cols1}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v0}\PY{p}{,}\PY{n}{n0}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v1}\PY{p}{,}\PY{n}{n1}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v2}\PY{p}{,}\PY{n}{n2}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign1}\PY{p}{:} \PY{k}{True}

\PY{n}{q2}\PY{p}{:} 
\PY{n}{cond2}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0} \PY{p}{)} 
\PY{n}{cols2}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v0}\PY{p}{,}\PY{n}{n0}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v1}\PY{p}{,}\PY{n}{n1}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v2}\PY{p}{,}\PY{n}{n2}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign2}\PY{p}{:} \PY{k}{True}
\end{Verbatim}


==> code/r2.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} 
\PY{n}{cond1}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{n}{v2} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{o}{!}\PY{n}{n2} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0}\PY{p}{)} \PY{p}{)} 
\PY{n}{cols1}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v3}\PY{p}{,}\PY{n}{isN3}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign1}\PY{p}{:} \PY{k}{True}

\PY{n}{q2}\PY{p}{:} 
\PY{n}{cond2}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0} \PY{p}{)} 
\PY{n}{cols2}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v4}\PY{p}{,}\PY{n}{n4}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign2}\PY{p}{:} \PY{k}{True}
\end{Verbatim}


==> legacy.tex <==

Machine learning and deep learning become popular methods for cardinality estimation \cite{ortiz2019empirical}, but none of these studies discussed the distribution shift, a common and dangerous problem in machine learning, to the best of our knowledge.
Solving the distribution shift problem is an essential step to deploy ML-based CE techniques into real applications.

Distribution shift, a common problem in machine learning applications, is the scenario when the testing data distribution differs from the training data distribution.
In CV, NLP, and other AI domains,  machine learning experts usually apply interactive learning, active learning, and online learning to resolve distribution shift problem.
In recent years, generative methods, such as Generative Adversarial Networks (GANs), also gains popularity  methods to synthesize additional data to improve model robustness.

Distribution shift in ML-based database systems is slightly different from shifts in traditional AI applications, which has some new challenges.
For example, in supervised cardinality estimation, DB systems usually requires the ML model to address distribution shifts automatically within a few minutes or even a few seconds.
In previous studies, researchers usually focus on the case that abundant real predicates already exists, but in reality the predicate acquisition rate (aka incoming rate) is usually various and unknown.

Some prior work uses fine-tuning or re-training to address the distribution shift problem. However, these methods need enough real data to achieve a satisfiable result.

So, we leverage generative methods to solve the distribution shift problem.
In this work, we 
(1) show that distribution shift is a severe problem to generalize machine learning-based approach for database management;
(2) create AdaP (Adapt Predicates shifts) system to mitigate distribution shift problem in cardinality estimation; and
(3) conduct empirical experiments to validate the robustness and limitation of the proposed AdaP system.

\section{Background}
\subsection{ML Methods for Cardinality Estimation}

\subsection{Predicate Representation}
Following LM's \cite{dutt2019lm} approach  for the single table experiment, the predicate $q$ has the form of $(l_1, l_2, ..., l_m, u_1, u_2, ..., u_m)$, where $l$ represents lower value, $u$ represents upper value, and table $T$ contains $m$ columns. 
It follows the template ``SELECT COUNT(*) FROM T WHERE $c_1 >= l_1$ AND $c_2 >= l_2$ AND ... AND $c1 <= u_1$ AND ... $c_m <= u_m$".

\subsection{The Impact of Distribution Shift}

On the other hand, GAN also receives criticisms on its training process because GAN does not necessarily converge to global Nash equilibrium \cite{heusel2017gans}. 







\section{Method: AdaP}
\label{sec:method}


\subsection{System Overview}
\label{sec:overview}
The proposed machine learning pipeline,  as shown in Figure \ref{fig:sys_overview}, contains the pre-trained machine learning model, an observation pool, a ground truth annotator, a synthesizer, and an active learner.

\textbf{Training a ML-based CE Model:}
for a static large database $B$, a machine learning system would randomly generate a few thousands workloads and acquire their ground truth cardinalities to train a CE model (e.g. similar in \cite{mscn,lm}, etc.) These workloads and their ground truth are stored in the observation pool, and they are used to train the machine learning model. When the machine learning model is well trained by using these randomly generated workloads, it is deployed to serve as a cardinality estimator.


\textbf{Inference Clients' Workload:}
when a client (either human or another system) request the cardinality estimator to approximate the cardinality for a given workload, the ML-based estimator can evaluate the workload within a few milliseconds (i.e. 2 ms in our empirical experiment, see Section \ref{sec:results}).
All clients' workloads are stored in an observation pool for future reference.

\textbf{Fine-Tune During Idle Time:}
when the system is in idle (e.g. after using the ML model to answer clients' requests), the system can fetch ground truths for unlabelled workloads in the observation pool.
Then, the system can fine-tune its machine learning models based on the newly acquired ground truth. 

\textbf{Detecting Distributional Discrepancies:}
The randomly generated workloads could be different from clients' workloads (e.g. Figure \ref{fig:dist_compare}), which is a common problem in all machine learning systems.

Now, there are two different scenarios:
(1) when there are too few clients' requests, the system does not have enough workloads to fine-tune the CE model;
(2) when there are too many clients' requests, the system has too much workloads to get ground truth labels.

\textbf{Case 1: Not Enough Real Workloads for Fine-Tune:}
for most large-scale database, clients would usually query a workload occasionally (e.g. only several times in a day for an employee management system in a small company). 
Generating New Workloads


\textbf{Case 2: Too Many Workloads in Observation Pool:}
when the incoming workload is relative large (e.g. several workloads within a few seconds for a shopping website), the system might have insufficient budget to acquire ground truth cardinalities. In this case, selecting the most useful Workloads from the observation pool could be more beneficial to fine-tune the machine learning model. 



The proposed AdaP system,  as shown in Figure \ref{fig:sys_overview}, can handle the distribution shift problems when there are too many or too few workloads.
It contains four components: ML-based estimator, workload synthesizer, active learner,  and ground truth annotator.
The ML-based estimator can be any gradient-based neural networks such as \cite{dutt2019lm, mscn}. 
The synthesizer is a Generative Adversarial Network (GAN) model that can learn real workloads' distribution.
The active learner uses classic unsupervised learning approaches to reduce redundancies and select valuable data for labelling.
The ground truth annotator is responsible to communicate with DBMS and provide ground truth to fine-tune the estimator.

In the following sections, we will focus on synthesizer and active learner, which provide adaptation functionality for the AdaP system. The ML-based estimator is similar to the ones in the previous literature, and it can be replaced by any blackbox ML models.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/system_overview.PNG}
    \caption{
    System Overview
    }
    \label{fig:sys_overview}
\end{figure}





\subsection{Synthesizer}
In many scenarios, a database would only be queried for a few times for a given hour. 
Hence, the system may need to wait for a long time to acquire enough real workloads to fine-tune the estimator to resolve distribution shift problem.
When the number of real workloads is insufficient to fine-tune machine learning-based cardinality estimators, the Synthesizer, which is based on Generative adversarial network (GAN), will synthesize additional real-alike workloads for labelling to mitigate the data-hunger problem.
Different from the classic GAN in machine learning, the proposed Synthesizer can learn both the prior, posterior, and joint probability distribution for the training and testing sets in real-time; hence, it have the potential to generate better workloads than the classic GAN. 
In this section, we first introduce the classic GAN approach, and then introduce our specially designed Synthesizer, which is based on GAN, for the adaptation task.
% {\color{red}Add Ablation? If yes, we may need to explain why the traditional GAN perform even worse than baselines (hard mining).}


% Generative adversarial network is based on previous generative methods in machine learning: modular learning \cite{ballard1987modular} tackles the encoder problem, the wake-sleep algorithm and the Helmholtz machine \cite{hinton1995wake} unify recognition and generation together, the auto-encoder model then applies for dimension reduction \cite{hinton2006reducing}, and auto-encoding variational Bayes and variational auto-encoders \cite{kingma2013auto} can efficient infer and learn directed probabilistic models.


Designing and training GAN are harder than training standard deep supervised learning models. Researchers need to avoid mode collapse and evaluate the convergence when training a GAN system. 
Most database systems requires real-time performance for its machine learning models, not only including the inference time but also the training time. Unfortunately, training a GAN system usually requires several minutes or even hours in deep learning applications.
Moreover, traditional unsupervised learning applications often do not require prior knowledge of the underlying distribution, but solving the dataset adaptation problem requires the understanding toward both the prior and posterior distribution of testing queries.
Hence, training a standard GAN could not fully solve the dataset shifting problem in database management systems.


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.35\textwidth]{fig/gan_part.PNG}
    \caption{ GAN for synthetic workloads. Each row represent one workload in the matrix. For the input workload matrix (green), the last column (dark green) represents ground truth cardinality. }
    \label{fig:gan_part}
\end{figure}

Our model needs to learn both the prior and posterior shifts. 
The prior distribution is $\mathds{P}_{train}(y)$ for the training set and 
$\mathds{P}_{test}(y)$ for the testing distribution, where $y$ is the labels (i.e. ground truth cardinality) in the machine learning problem.
The prior distribution represents the knowledge toward the data before observing it. On the other hand, the posterior distribution is a conditional probability distribution given observed features such that $\mathds{P}_{train}(y|x)$ for the training set and $\mathds{P}_{test}(y|x)$ for the testing set. In our dataset adaptation setting, the posterior distribution for the training set and testing set is the same, which is  $\mathds{P}_{train}(y|x) = \mathds{P}_{test}(y|x)$, because given the same feature, the underlying ground truth cardinality would stay the same for the training and testing time.


Different from traditional GAN that only learns data distribution, the discriminator in our system will learn 
the data distributions
(i.e. $\mathds{P}_{train}(x)$,
$\mathds{P}_{real}(x)$, and
$\mathds{P}_{fake}(x)$)
and the joint distribution 
(i.e. $\mathds{P}_{train}(x,y)$,
$\mathds{P}_{real}(x,y)$, and
$\mathds{P}_{fake}(x,y)$). 
Learning these distributions can provide better synthesized workloads and hence expedite the adaptation process for the machine learning-based cardinality estimator.

Define $D$ as the discriminator and $G$ as the generator. 
The discriminator $D$ will distinguish whether the incoming data/cardinality comes from the training dataset, testing dataset, or fake dataset.
For an input workload $q$, $D(q, y) \in [0, 1]^3$ represents the probability $q$ is a training, testing, or fake workload. Denote $D(q, y)_i$ as the probability that $q$ is in class $i$ so that $\sum\limits_{i=0}^2 D(q, y)_i = 1$. 
$\hat{v}_i$ is a one-hot vector represents the class of workload $q$. For instance, if $q$ is a real workload, $\hat{v} = [0, 1, 0]$. 

The generator $G$ needs to synthesize real-like workloads (without ground truth cardinality).
Given an input vector $c\in \mathds{R}^m$ and a random vector $z \in \mathds{R}^r$, the generator will generate $\delta_u \in \mathds{R}_+^m$ (upper range) and $\delta_l \in \mathds{R}_+^m$ (lower range) to synthesise a workload as $(c_1 - \delta_{l_1}, c_2 - \delta_{l_2}, ..., c_m - \delta_{l_m}, c_1 + \delta_{u_1}, ..., c_m + \delta_{u_m})$. As the formula shows, the input $c$ is a ``center" for the output workload and $z$ is random seeds for the generation.


Consistent with traditional GAN, the proposed discriminator and  generator will train to optimize $\min\limits_{G}\max\limits_{D} V(D, G)$, where $V(D,G)$ is defined as:

\begin{align}
\begin{split}
    V(D, G)  = & \mathds{E}_{q \sim p_{data_{test}}(q)}\sum\limits_{i=0}^2 log(D(q, y)_i)\hat{v}_i \ \ + \ \  \\
    & \mathds{E}_{q \sim p_{c, z}(c, z)} log(1- D(G(c, z))_1, y)
\end{split}
\end{align}

As discussed, the proposed system can learn joint probability for $\mathds{P}(x, y)$ and $\mathds{P}(y)$. However, we could not fetch the ground truth for all generated workloads during the training process. So, we use ``-1" as a flag to represent NaN (unknown cardinality) for the generated workloads. To avoid the discriminator to bias towards the ``-1" flag, we would randomly replace ground truth cardinality for the workloads (with known cardinality) in the training and testing distribution. Hence, when we provide $y = -1$ as a feature for the discriminator, the discriminator also needs to learn and make predictions solely based on the workload distribution without cardinality (i.e. $\mathds{P}_{real}(x)$).

In addition, we apply the following strategies to improve the robustness of the proposed synthesizer.

\textbf{Convergence and Early Stopping:}
The generator and adversarial are playing zero-sum mini-max game together. When they reach Nash equilibrium, the training process can be stopped early to save computational time. Nevertheless, it is still an open problem how to define and assess whether a GAN system reached equilibrium or not. 

The GAN system will utilize previously generated workloads into training to augment its set to avoid overfitting and mode collapse.
Similar to \cite{fan20relational}, AdaP uses smaller discriminator than generator to avoid overfitting the discriminator. The discriminator and generator in AdaP have the same depth, but the discriminator is twice narrower than the generator in width.

During the fine-tuning time, the synthesizer will stop training when both the generator and discriminator have over 0.6 score such that: (1) the discriminator has over 60\% F-1 score for 3-way classification, and (2) over 60\% of generator's synthetic workloads are misclassified as testing workloads by the discriminator. So, the system has another gate to avoid overfitting, which can also reduce the training time if the system can quickly converges to equilibrium.

\textbf{Convergence Gate:}
If the convergence criterion is not reached after a certain number of epochs, the generator and discriminator could not reach the equilibrium case. This problem could be occurred when there are too few real predicates.
In this case, the Synthesizer will randomly generate additional queries by applying a simple ad-hoc algorithm \ref{algo:ad-hoc-generation}.
From our observation, this special failure only occurs ??\% of the time.



\textbf{Variety of Synthetic workloads:}
one common problem for GAN is mode collapse, when the generator only generate similar workloads disregard what the input $c$ and $z$ are. In the last few years, many studies (e.g. Unroll GAN \cite{metz2016unrolled}, Wasserstein Loss \cite{arjovsky2017wasserstein}, VEEGAN \cite{srivastava2017veegan}, etc.) design different approach to solve this problem. In this study, the generator outputs $\delta_l$ and $\delta_u$ around the random center $c$, which guarantees the resulting workload is more various by design.
An extreme case is when none of the testing workloads are around center $c$, then the discriminator could easily reject this generated workload.
During inference time, the AdaP system will filter all generated workloads and their cardinalities by discriminative sampling as described below.


\textbf{Discriminative Sampling for Estimator Training:}
AdaP needs to use both the real data and augmented data to train the ML-based estimator.
The augmented samples are weighted random sampled from the augmentation pool, where the weights are calculated from the discriminator.
By this design, AdaP can use the power from the latest discriminator to evaluate augmented workloads generated in all times. 
The latest discriminator has seen more workloads than few hundreds seconds ago, and hence is more robust to judge the augmented workloads.
So, even if the generator could not generate high-quality workloads in the first few iterations, the discriminator knows to discard these low-quality workloads in later iterations.

\subsection{Active Learner}
When the system has abundant of real workloads coming per second, the system do not need to generate synthetic workloads for training purpose. Instead, the system need to decide which workloads are valuable as new training data and then process these workloads to get ground truth. 
The AdaP utilize clustering algorithms to remove redundancies and sample from diverse sub-spaces. 


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\textwidth]{fig/al_part.PNG}
    \caption{ Active Learning to sieve valuable workloads for ground truth labelling }
    \label{fig:al_part}
\end{figure}


The system  will first apply Principle Component Analysis (PCA) to all workloads (including training and testing workloads) to reduce variance. 
AdaP use batch normalization so that the projected embeddings are normalized to have mean = 0 and standard deviation = 1.
Then, the system will apply Gaussian Mixture model and cluster the embeddings to several smaller partitions. 
At last, the system will survey each partition from the Gaussian Mixture model, and randomly sample from partitions with less known (i.e. with more uncertainty) workloads.


\textbf{Embeddings:}
we decide to use PCA to calculate the workload embedding because of its speed and exactness.
The embedding task is easier than generative tasks described in the previous subsection, which can be achieved by use linear methods.
Some recent natural language studies (e.g. \cite{levy2014neural}) also suggest that traditional Single Value Decomposition (SVD) method is on par with many modern embedding approaches for word similarity task.
In this study, we also examined multi-layer autoencoder and variational autoencoder, but PCA is superior than these neural-based approaches if we constraint the computation costs.
The embeddings are normalized for the clustering algorithm below. 
% {\color{red} Do we need ablations? I can run autoencoder experiments after finishing all other AL experiments.}

\textbf{Clustering:}
AdaP system uses Gaussian Mixture Model (GMM) and expectation-maximization algorithm for clustering because it can perform probabilistic analysis and provide numerical value so that AdaP can quantitatively evaluate the performance of clustering.
% TODO: introduce more about GMM. Maybe 2 - 4 sentences about mean, variance, P(y|x), etc.
In our experiments, we set the initial number of clusters to 100, but most of these clusters might be ignored by GMM when fewer number of clusters provide good separation for workload embeddings; so, the number of initial clusters is not important and will be overrode automatically over time.
% We fine-tune the GMM as the number of incoming workloads increases. 
Define the clustering score, which ranges from 0\% to 100\%, as the mean likelihood for all workloads under the current GMM.
When GMM reaches at least 90\% score, AdaP system will accept the GMM's clustering results as valid and perform further process (i.e. selection through weighted sampling); otherwise, AdaP will reject the GMM and just perform uniform random sampling from the real workloads pool.

\textbf{Sampling workloads from Clusters:}
The proposed active learning approach in AdaP system balance exploration and exploitation via weighted random sampling from each clusters. 
In addition, AdaP will find and exploit more on hard examples (with higher loss) while fine-tuning its ML-based estimator.



\subsection{Implementation Details}

\textbf{Threads and Con-currency}
AdaP uses a separate thread for each of the components (i.e. base ML estimator, generative synthesizer, active learner, ground-truth annotator) so that each of these agent would not block each other. 
We sum up the total CPU time for these different threads to calculate the computation costs.



\textbf{AdaP Parameters}

\section{Empirical Experiments} % 1 page

\subsection{Datasets}

For single table CE experiments, we use the following datasets:
\begin{itemize}
    \item Lineitem
    \item HIGGS
    \item Poker
    \item PRSA
\end{itemize}

For join CE experiments, we use the following datasets:
\begin{itemize}
    \item IMDB
    \item Credit
    \item TPC-H
    \item HIGGS
\end{itemize}

\subsection{Predicates Simulation}

\textbf{Data-centric}

\textbf{Random-centric}

\textbf{Row-centric}

\textbf{Multi-Row-centric}

\textbf{Density-centric}


The cold predicates are generated from data-centric and random-centric method, which is an effective way to cover the space \cite{dutt2019lm}.
The real predicates are generated from row-centric, multi-row-centric, and density-centirc methods.
We also apply random masks to real predicates and ensure their cardinality is within 2\% of the table length.

As shown in Figure \ref{fig:dist_compare}, even if the training and testing distributions have big portion of overlaps, some regions in the testing distribution are still not fully covered by the training distribution.



\subsection{Metrics}
We use GMQ (geometric-mean of Q-error) as the metric to evaluate a CE model. 


Time to reduce half errors (TRH) is used to evaluate how fast a machine learning system can adapt to a distribution shift.


\subsection{Targeting ML Models}

\textbf{Single Table CE Model:} we use LM as a single table CE model. For simplicity, all single table experiments use 64KB model as the base estimator.

\textbf{Join CE Model:}
In this study, we combine LM \cite{dutt2019lm} and MSCN \cite{mscn} to create a more memory-efficient join CE model.
As shown in Figure \ref{fig:lm_join}, {\color{red} TODO ...}

The input for the Synthesizer for join task contains: random seed, some real predicates, and random lower/upper bounds.  {\color{red} TODO ...}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.25\textwidth]{fig/LM_Join.png}
    \caption{ Feature representation for our join model.}
    \label{fig:lm_join}
\end{figure}

\subsection{Experiment Settings}


\subsubsection{Baseline Methods}

\textbf{Standard Fine-tune:}

\textbf{Hard-example Mining:}

\textbf{Ad-hoc Data Augmentation:}


\begin{algorithm}[h]
\SetAlgoLined
\LinesNumbered
\KwIn{A set of real predicates $S$, \\ Dimension of the dataset is $d$}
% \KwOut{Optimized Neural Network $f$}
% \KwData{Training data $X$, training labels $y$}
\KwOut{A new predicate $x$}
Randomly select $s_1 \in S$;\\
Randomly Select $s_2 \in S$;\\
Set $x = s_1$;\\
\ForEach{$i \in [0, 1, ..., d]$}{ 
    \If{Random Coin Head}{
        $x$'s dimension $i$ = $s_2$;
    }
}
$x = x + \mathcal{N}(0, \sigma)$;
\caption{Ad-hoc Predicate Generation}
\label{algo:ad-hoc-generation}
\end{algorithm}

\section{Results} % 3 pages
\label{sec:results}

\subsection{Performance Improvement}

\subsection{Cost}


==> sections/8acknowledgments.tex <==
\section{Acknowledgments}
CSC, AWS credit, DASLab funding.

==> system.tex <==
\section{System design}
\label{sec:method}



\begin{figure}[t!]
    \centering
    \includegraphics[width=0.88\linewidth]{fig/system.png}
    \caption{
    Overview of the {\name} system.
    }
    \label{fig:sysoverview}
\end{figure}


We propose a system {\name} which handles data and workload shifts in a unified manner given a previously trained CE model. We describe in this section our system design and different use cases.  

\vspace{0.05in}
\noindent\textbf{System overview.} Figure \ref{fig:sysoverview} showcases our system architecture, with the following components: 

\begin{itemize}
\item \emph{The query pool} is the heart of {\name} for maintaining tuples of $\{{\tt q},{\tt gt},z,l,l', c'\}$, in which {\tt q} stands for a query predicate; {\tt gt} is the ground truth label.  $l$ and $l'\in\{{\tt train}, {\tt test}, {\tt gen}\}$ depicts the actual label and prediction from the discriminator $\mathbb{D}$ for a query predicate being drawn from the original training workload {\tt q}*, the test workload {\tt q} or generated workload  ${\tt q}_{\tt gen}$ respectively. $c'$ is the confidence scores for the prediction. $z$ is the learned embedding of the query predicate. 

\item \emph{The CE model} $\mathbb{M}$ is previously trained offline and is the model that {\name} aims to improve. The CE models that {\name} can use include LM[] and MSCN[] in our experiments. 

\item \emph{The picker} $\mathbb{P}$ borrows the idea from active learning [] and exposes \texttt{pick}() that takes a batch of query predicates as input and rank them in terms of usefulness to the CE model.   

\item \emph{The generator} $\mathbb{G}$ uses \texttt{gen}() to synthesize queries. It is trained in a GAN fashion together with $\mathbb{D}$, the discriminator that exposes \texttt{dsc}(), so that generated queries play an adversarial game with $\mathbb{D}$. We denote $s_{\tt gen}$ as the rate of queries generated. More details follow in Section~\ref{sec:individual}.
\end{itemize}

There are a few auxiliary components. The \emph{input queue} $\mathbb{I}_{\tt test}$ injects queries from the test workload into our system; we use $s_{\tt query}$ for the injection rate. The \emph{training queue} $\mathbb{I}_{\tt train}$ injects queries from the original training workload that is used for building $\mathbb{M}$. The \emph{annotator} $\mathbb{A}$ loads a query predicate from $\mathbb{P}$ and queries the data for ground truth labels; it can be custom code or a DBMS. We denote $s_{\tt gt}$ as the rate of queries that can be annotated by \texttt{anno}().  The \emph{encoder} $\mathbb{E}$ is a learned embedding upon the query predicates and exposes {\tt embed()}. Section ? describes the individual modules.
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table}[t]
\begin{footnotesize}
\centering
\begin{tabular}{l|c|c|c|c} 
Use case & {\tt use}\_$\mathbb{G}$ & {\tt use}\_$\mathbb{P}$ & {\tt use}\_$\mathbb{E}$ & Update $\mathbb{M}$ \\\hline
1. $s_{\tt gt}, s_{\tt query} \ge t$ & $\times$ & $\times$ & $\times$ & $\checkmark$ \\
2. $s_{\tt query}<t$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
3. $s_{\tt gt}\le t<s_{\tt query}$ & $\times$ & $\checkmark$ & $\times$  & $\checkmark$\\
\hline
\end{tabular}
\caption{Different use cases considered by {\name}. \label{t:case}}
\end{footnotesize}
\end{table}

\vspace{0.05in}
\noindent\textbf{System runtime. } {\name} runs in minibatches and calls different modules for maintaining the pool. Algorithm \ref{alg:qgan} describes the system runtime in each minibatch. Specifically, inputs to each minibatch include a set of query predicates \texttt{q} and corresponding cardinality \texttt{gt} from the test workload; {\tt push}() injects these records into the pool. Next, {\name} computes embeddings of query predicates using $\mathbb{E}$, synthesizes query predicates using $\mathbb{G}$ and picks useful queries using $\mathbb{P}$ as described in Table \ref{t:case}. Three important variables $n_{\tt train}, n_{\tt test}$ and $n_{\tt gen}$, depicting the numbers of examples from different workloads to update $\mathbb{M}$, will be discussed later in this section. The models are updated using the augmented workload $\{q, gt\}$ remaining in the pool after applying the picker. The final outputs of {\name} in a minibatch are the updated $\mathbb{M}$ together with the updated learned models. %It is easy to see that the generator and the picker can be switched off in different use cases; meanwhile, each of them exposes \texttt{update}() as will be discussed shortly. 
Note that a large portion of the learned models can be parallelized; we use an {\tt async} keyword for an asynchronous invocation.

\begin{algorithm}[t!]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{\{\texttt{q}, \texttt{gt}\} from $\mathbb{I}_{\tt test}$, $\mathbb{M}$ and learned models from the previous minibatch.}
%\emph{Compute embedding:}\\
{\tt push}(\{{\tt q}, {\tt gt}, $l$={\tt test}\})\;

{\tt async} \{ $\texttt{gt}\leftarrow\texttt{anno}(\texttt{q|gt=-1}$) \textbf{for} {\tt record} \textbf{in} {\tt Pool}; \}\\

\textbf{if} use\_$\mathbb{G}$:\\

\hspace{0.25in}//\emph{Invoke learned models asynchronously.}

\hspace{0.25in}{\tt async} \{ $\texttt{z}\leftarrow\texttt{embed}({\tt q, gt}|z=\varnothing$)  \textbf{for} {\tt record} \texttt{in} {\tt Pool}; \}\\

\hspace{0.25in}{\tt async} \{ $l',c'\leftarrow{\tt dsc}(z|l={\tt gen})$  \textbf{for} {\tt record} \texttt{in} {\tt Pool}; \}\\ 

\hspace{0.25in}\textbf{while} $n_{\tt g}${-}{-}: //\emph{Update GAN.}\\

\hspace{0.5in}$\texttt{q}^{*}_{\tt gen}\leftarrow\{\texttt{gen}(z|l={\tt test}\}, n$*$)\}$\; 

\hspace{0.5in}Compute $\mathcal{L}_{\tt GAN}$ using ${\tt q}_{\tt gen}*, {\tt q}\in{\tt Pool}$\;

\hspace{0.5in}$\mathbb{G}, \mathbb{E},\mathbb{D}\leftarrow\texttt{update\_GAN}(\mathbb{G},\mathbb{E},\mathbb{D}, \mathcal{L}_{\tt GAN});$ \\

\hspace{0.25in}//\emph{Update learned models.}\\

\hspace{0.25in}Compute $\mathcal{L}_{\tt AE}$ using ${\tt q}\in{\tt Pool}$; \\

\hspace{0.25in}$\mathbb{G},\mathbb{E},\mathbb{D}\leftarrow{\tt update\_multi\_task}(\mathbb{G},\mathbb{E},\mathbb{D}, \mathcal{L}_{\tt AE}+\mathcal{L}_{\tt GAN})$\;

\hspace{0.25in}//\emph{Generate queries.}\\

\hspace{0.25in}$\texttt{q}_{\tt gen}\leftarrow\{$ $\texttt{gen}(z|l={\tt test}, n_{\tt gen'})$ $\}$;\\ 

\hspace{0.25in}{\tt push}(\{{\tt q}$_{\tt gen}$, {\tt gt}=-1, $l$={\tt gen}\}); \\

\hspace{0.25in}$\texttt{pick}(l={\tt gen}, n_{\tt gen})$\;

\textbf{if} use\_$\mathbb{P}$:\\
\hspace{0.25in}$\texttt{pick}(l\in\{{\tt train,test}\}, n_{\tt train}, n_{\tt test})$\;

{\tt sync}(); $\mathbb{M}\leftarrow\texttt{update}(\mathbb{M}, \{\texttt{q,gt}\}\in{\tt Pool})$\;

%\hspace{0.25in}\textbf{if} use\_$\mathbb{P}$: $\mathbb{P}\leftarrow\texttt{update}(\mathbb{P},\Delta)$\;
\Output{Updated model $\mathbb{M},\mathbb{G},\mathbb{D},\mathbb{E}$ for the next minibatch.}
\caption{{\name} procedures in a minibatch. \label{alg:qgan}}
\end{algorithm}



\vspace{0.05in}
\noindent\textbf{Use cases.} 
The {\name} execution pipelines vary in different use cases depending on $s_{\tt query}$, $s_{\tt gt}$ and $t$, where $t$ depicts the rate of annotated queries that are necessary to obtain a robust model; we discuss later how to estimate this threshold. Table \ref{t:case} describes different use cases and configurations in {\name}. We believe these configurations already cover most practical use cases in different data and workload shift problems. In general, {\name} (1) ${\tt use}\_\mathbb{G}={\tt use}\_\mathbb{E}=s_{\tt query}<t$: {\name} uses the generator $\mathbb{G}$ and the encoder $\mathbb{E}$ whenever there is not enough queries to reach $t$ so that more training queries need to be synthesized; (2) ${\tt use}\_\mathbb{P}={\tt use}\_\mathbb{G}\cup(s_{\tt gt}<s_{\tt query})$: {\name} uses the picker $\mathbb{P}$ whenever annotation cannot keep up or whenever the generator is used. 


\vspace{0.05in}
\noindent\emph{Cracking data shift.} When data shifts $D\rightarrow D'$ and workload does not change, labels from the training queries are outdated and we must re-compute them. In such a scenario, there are enough queries than necessary but ground truth computation cannot keep up for a fast adaptation $s_{\tt gt}\le t<s_{\tt query}$ ({\tt Case3} in Table \ref{t:case}). Hence, {\name} disables the generator $\mathbb{G}$ and uses the picker $\mathbb{P}$ only. To accelerate model adaptation given a limited cost budget, $\mathbb{P}$ picks which queries are more useful, annotate these queries and updates $\mathbb{M}$ accordingly.   

\vspace{0.05in}
\noindent\emph{Cracking workload shift.} When the data keeps unchanged but the workload shifts $X\rightarrow X'$, we note different use cases of {\name}. 
(1) {\tt Case1} in Table \ref{t:case} demonstrates a scenario when both queries and ground truth are adequate; hence {\name} shuts down the generator and the picker and updates the model $\mathbb{M}$ using the available queries and ground truth. 
(2) {\tt Case2}: when the workload begins to shift and there is inadequate test queries from observation ($s_{\tt query}<t$), {\name} enables the generator $\mathbb{G}$ to fill the gap between $s_{\tt query}$ and $t$; meanwhile the picker also kicks into action to find useful queries withing the pool.  
(3) {\tt Case3} shows a scenario when there is adequate queries, but ground truth computation cannot keep up. Examples of this use case include in a query optimizer when what-if queries are issued but there lacks ground truth labels for them.  As in the data shift case, {\name} uses the picker $\mathbb{P}$ only so as to rigidly spend the annotation budget.

\vspace{0.05in}
\noindent\noindent\emph{Combined scenario.} When both data and workload shift, {\name} considers a combination of {\tt Case2} and {\tt Case3} in the workload shift case. There are not enough queries while labels from the training workload are also outdated; {\name} uses all learned models. 

\subsection{Using Individual Modules}\label{sec:individual}
Here, we describe in detail the design and implementation of individual modules used in our system. The function calls, inputs and outputs of each module is shown in Figure~\ref{fig:sysoverview}. 

\vspace{0.05in}
\noindent\textbf{The query pool} is an in-memory data structure that maintains necessary training data, cardinality and query labels in $\{{\tt q},{\tt gt}, z,l,l',c'\}$ tuples. {\name} initializes the query pool with $\mathbb{I}_{\tt train}$ from the original training workload. Each $\{{\tt q}$*$, {\tt gt}$*$\}$ tuple from $\mathbb{I}_{\tt train}$ creates a record in the query pool with empty $z, l',c'$ and $l={\tt train}$. In Algorithm~\ref{alg:qgan}, $\mathbb{I}_{\tt test}$ from the test workload is injected into the query pool in a new minibatch; similarly we insert a record in the query pool with $l={\tt test}$. The generator $\mathbb{G}$, when necessary, injects new records with ${\tt q}_{\tt gen}$ into the query pool with $l={\tt gen}$ and {\tt gt}=-1. Meanwhile, the picker $\mathbb{P}$ filters the query pool by keeping only useful queries before they are used to update the CE model $\mathbb{M}$. {\name} fills the missing record fields using different {\name} modules ($\mathbb{A}$, $\mathbb{E}$ and $\mathbb{D}$) in an asynchronous manner. 

\vspace{0.05in}
\noindent\textbf{The CE Model $\mathbb{M}$} is used as a black box and predicts cardinality given a query predicate: $${\tt q}\rightarrow\mathbb{M}\rightarrow {\tt card}.$$ {\name} requires exposure to only the \texttt{update()} API from the model which either re-trains or fine-tunes the model given a set of training examples $\{{\tt q'},{\tt gt'}\}$ from the query pool. {\name} aims at improving the CE model without changing the model design; for models that require additional input, such as MSCN which takes a bitmap as input, {\name} does not break the contract and such additional input can be from a side stream. Whether re-training or fine-tuning depending on individual models. For example, models based on neural networks are iteratively trained and supports fine-tuning, while tree-based models have to be re-trained. 

We note that {\name} requires an initial input of $\mathbb{M}$ that is previously trained offline using $\{{\tt q}$*$, {\tt gt}$*$\}$ which formulates $\mathbb{I}_{\tt train}$ in {\name}. {\tt gt}* can be reused in workload shift cases but has to be re-computed in a data shift. Featurization of {\tt q} also depends on the specific model; for example in LM, ${\tt q}=\{{\tt low}_1,..,{\tt low}_d,{\tt high}_1,..,{\tt high}_d\}$ is a vector containing low and high range checks of the query predicate. Such featurizaiton is used among different {\name} modules and hence {\name} simply inherits the original featurization for $\mathbb{M}$.

\begin{table}[t]
\begin{footnotesize}
\centering
\begin{tabular}{c|c|c|c}
Layer & Encoder $\mathbb{E}$ & Generator $\mathbb{G}$ & Discriminator $\mathbb{D}$ \\ \hline
1 & Fully Conn. 128 & Fully Conn. 128 & Fully Conn. 64 \\
2 & RELU activation & RELU activation & RELU activation\\
3 & Dropout(0.3) & Dropout(0.3) & Dropout(0.3)\\
4 & Fully Conn. 128 & Fully Conn. 128 & Fully Conn. 1\\
\hline
\end{tabular}
\caption{Model specifications.\textcolor{red}{Update}}
\label{t:model}
\end{footnotesize}
\end{table}  

\vspace{0.05in}
\noindent\textbf{The Encoder $\mathbb{E}$} is a learned embedding that transforms a query predicate together with its ground truth cardinality label into a compact representation: $${\tt embed(}{\tt q}, {\tt gt}): {\tt q}, {\tt gt} \rightarrow\mathbb{E}\rightarrow z.$$ {\name} uses the learned representations of query predicates so as to improve the effectiveness of subsequent learned models.  {\tt gt}=-1 by default in case ground truth labels are unavailable from a workload.  $\mathbb{E}$ uses a simple NN and is trained with records in the pool with and without {\tt gt} labels.  The model detail is illustrated in Table \ref{t:model}. %Notably, $\mathbb{E}$ is trained on \{{\tt q}, {\tt gt}\} pairs whenever ground truth labels are available, since distributions of both {\tt q} and {\tt gt} can shift in the test workload. 
 
\vspace{0.05in}
\noindent\textbf{The Generator $\mathbb{G}$} consumes the compact representation of a query predicate and produces a new query predicate: $${\tt gen}(z,n): z+\epsilon\rightarrow\mathbb{G}\rightarrow {\tt q}_{\tt gen},$$  where $n$ is the number of queries generated, $\epsilon \sim \mathbb{N}(0, \sigma^2)$ is a random Gaussian noise with standard deviation $\sigma$ that equals to the standard deviation of $z$. $\mathbb{G}$ is a simple NN that is not wildly different than other learned models in our system (Table~\ref{t:model}). However, unlike other NN modules, $\mathbb{G}$ is trained together with the discriminator $\mathbb{D}$ using an adversarial loss to formulate a GAN -- details follow in in Section ?. On the other hand, $\mathbb{G}$ generates query predicates based on existing ones in the pool. We consider this appropriate and perhaps also necessary, since query predicates can be drawn from a high-dimensional space; generating from a fully random seed is less likely to land into the real test workload. We will show in our experiments that using a learned generator here also outperforms manually adding noise upon existing queries.   

\vspace{0.05in}
\noindent\textbf{The Discriminator $\mathbb{D}$} is another NN that takes the representation of a query predicate as input and predicates a label for the query predicate being generated, pulled from test workload or from the original training workload:  $${\tt dsc}(z): z\rightarrow\mathbb{D}\rightarrow l'\in\{{\tt gen},{\tt test},{\tt train}\}, c'.$$  As shown in Algorithm \ref{alg:qgan}, $\mathbb{G}$ and $\mathbb{D}$ need to be updated in each minibatch before actual generation. The $l'$ labels are used in the training so that $\mathbb{D}$ can successfully differentiate the generated queries. 

Table~\ref{t:model} demonstrates the model design of $\mathbb{G}$ and $\mathbb{D}$. The goal here is simplicity and generalizability. In our experiments we will show that such design already cover many of the test scenarios. For cases when these models become difficult to learn any useful information, \textcolor{red}{using different models} or increasing the model sizes can help. However, this is out of the scope of this paper and we defer to future work for model selection and hyper-parameter tuning. 

\cut{
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/picker.jpg}
    \caption{ Picker \textcolor{red}{Redraw} }
    \label{fig:picker}
\end{figure}}

\vspace{0.05in}
\noindent\textbf{The Picker $\mathbb{P}$} exposes {\tt pick}($c$, $n$) in which $c$ is an input condition and $n$ is the number of queries picked. It filters the records and finds those that can be more useful to the model $\mathbb{M}$. As shown in Algorithm~\ref{alg:qgan}, there are two use cases of $\mathbb{P}$. For generated query predicates with $l={\tt gen}$ (line 17), $\mathbb{P}$ keeps those with $l'={\tt test}$ labeled by $\mathbb{D}$ at high confidence. For the remaining records in the pool (line 19), we apply a stratified sampling over the embedding vectors $z$. Specifically, we first compute PCA eigenvectors among all $z$ vectors form the pool using SVD and reconstruct each $z$ into $d_{\tt pca}$ dimensions []. A Gaussian Mixture Model (GMM) [] is applied thereafter with a maximum number of clusters $n_c$ and merging threshold $\theta$; each record is replaced with the identifier for which Gaussian model it belongs to. Finally, a stratified sampling picks records among different GMM cluster ids. 

\subsection{Training Individual Modules}
There are three learned components in {\name}: the Encoder $\mathbb{E}$, the Generator $\mathbb{G}$ and the Discriminator $\mathbb{D}$. We formulate training these models as an end-to-end, multi-task learning problem as discussed in Algorithm~\ref{alg:qgan} and in the following. 


\vspace{0.05in}
\noindent\textbf{{\tt Task 1} Auto-encoder:} The first task is to train an auto-encoder that consists of the encoder $\mathbb{E}$ and the generator $\mathbb{G}$:  
$${\tt q},{\tt gt}\rightarrow\mathbb{E}\rightarrow z\rightarrow\mathbb{G}\rightarrow \hat{\tt q}.$$ 
Note that no random input $\epsilon $ is used here such that the auto-encoder is literally encoding and  reconstructing the input instead of generating new data. That said, the training goal of the auto-encoder is to minimize the reconstruction (L1) loss between the input query predicate and the recovered one: 
\begin{equation}
\mathcal{L}_{\tt AE}=|{\tt q} - \hat{\tt q}|.\label{eq:ae}
\end{equation}
Training the auto-encoder follows the standard approach []. During training (line 12), we use all records from the pool no matter if ground truth labels are available; {\tt gt}=-1 when ground truth labels are not immediately available. Doing so ensures that the encoder and the generator can generalize to all three cases (i.e., queries from the generator, the training workload or from the test workload).

\vspace{0.05in}
\noindent\textbf{{\tt Task 2} GAN:} The second task is to train the generator $\mathbb{G}$ together with the discriminator $\mathbb{D}$ in a GAN fashion []. More details are illustrated in Algorithm~\ref{alg:qgan} line 7-10 in which we show an iterative procedure; in each step, $\mathbb{G}$ generates a set of query predicates $q^{*}_{\tt gen}$ as described earlier and $\mathbb{D}$ distinguishes an input query predicate for belonging to $\{{\tt gen},{\tt test},{\tt train}\}$:
$$z+\epsilon\rightarrow\mathbb{G}\rightarrow{\tt q}^{*}_{\tt gen},-1\rightarrow\mathbb{E}\rightarrow z'\rightarrow\mathbb{D}\rightarrow l'.$$ 
The generator loss is defined by:
$$\mathcal{L}_{\tt gen} = {\tt CrossEntropy}(l', {\tt test}).$$
The goal here is to generate queries as close to the test workload as possible; in such a case the discriminator classifies the generated query as {\tt test}, despite that the actual label for generated queries are $l={\tt gen}$. A cross entropy ${\tt CrossEntropy}(p,q)=-\sum_{x\in X}p(x)\log q(x)$  is used here that follows an usual approach for training classifiers []. 

On the other hand, the discriminator is trained by classifying the generated queries as well as those existing ones from the pool (line 9 in Algorithm~\ref{alg:qgan}): 
$${\tt q},{\tt gt}\rightarrow\mathbb{E}\rightarrow z\rightarrow\mathbb{D}\rightarrow l_d.$$
The discriminator loss is defined by:
$$\mathcal{L}_{\tt discr} = {\tt CrossEntropy}(l,  l_d),$$
such that the discriminator should correctly identify which workload a given query predicate should belong to. Finally, the GAN loss is a combination of the generator and the discriminator losses: 
\begin{equation}\label{eq:gan}
\mathcal{L}_{\tt GAN}  = \mathcal{L}_{\tt gen} + \mathcal{L}_{\tt discr}.
\end{equation}
The training simultaneously optimizes $\mathcal{L}_{\tt gen}$ and $\mathcal{L}_{\tt discr}$ so that $\mathbb{G}$ and $\mathbb{D}$ play against each other and formulate a GAN. We note that unlike a classic GAN training in which a binary label of \{{\tt real},{\tt gen}\} is used,  here we use a three-class label of $\{{\tt gen},{\tt test},{\tt train}\}$. In workload shift cases, {\tt test} and {\tt train} represent different predicate distributions and in our experiments we showcase that introducing an addition class improves the generation and the adaptation. 
 

\vspace{0.05in}
\noindent\textbf{Multi-task learning.}  To train the learned components in {\name}, a multi-task loss function is used which consists of Eq.~\ref{eq:ae} and Eq.~\ref{eq:gan}:
\begin{equation}
\mathcal{L}  = \mathcal{L}_{\tt GAN}+\mathcal{L}_{\tt AE}.
\end{equation}
\noindent The training procedure is described in Algorithm~\ref{alg:qgan}. Specifically, we first run {\tt task 2} in line 7-10 and update $\mathbb{G}, \mathbb{E}, \mathbb{D}$ using only the GAN loss. Next, we run {\tt task 1} in line 12 and collect the auto-encoder loss using existing records in the pool. The auto-encoder loss and the GAN loss from the last iteration are merged (line 13) so as to update $\mathbb{E}$, $\mathbb{G}$ and $\mathbb{D}$ again. Finally,{\name} generates queries using the updated models (line 15). 
 
\begin{table}[t]
\begin{footnotesize}
\centering
\begin{tabular}{c|c}
Metric & Implication\\\hline
$t$ & \# of annotated queries needed for a robust model.\\
$s_{\tt query}$ & \# queries from $\mathbb{I}_{\tt test}$ injected into {\name} in a minibatch. \\\hline
$c_{\tt gt}$ & Cost to compute ground truth cardinality in a minibatch. \\
$c_{\tt Model}$ & Cost to update $\mathbb{M}$ in a minibatch. \\
$c_{\tt AE}$ & Cost to train {\tt task 1} and compute $\mathcal{L}_{\tt AE}$ in a minibatch. \\
$c_{\tt GAN}$ & Cost to train {\tt task 2} and compute $\mathcal{L}_{\tt GAN}$ in a minibatch. \\
$c_{\tt gen}$ & Cost to generate examples in a minibatch. \\
$c_{\tt pick}$ & Cost to pick examples in a minibatch.\\\hline
$n_{\tt train}$ & \# of examples from $\mathbb{I}_{\tt train}$ to update $\mathbb{M}$.\\
$n_{\tt test}$ & \# of examples from $\mathbb{I}_{\tt test}$ to update $\mathbb{M}$.\\
$n_{\tt gen}'$ & \# of examples generated by $\mathbb{P}$.\\
$n_{\tt gen}$ & \# of generated examples picked by $\mathbb{P}$ to update $\mathbb{M}$.\\\hline
$n_{\tt g}$ & \# of iterations used in training {\tt task 2}.\\\hline
\end{tabular}
\caption{Quantitative metrics used in {\name}}\label{t:param}
\label{t:param}
\end{footnotesize}
\end{table}  

\subsection{Training Corpus Composition and Cost Budgeting}
Table~\ref{t:param} lists the quantitative knobs used in {\name}. Some of them have been covered in prior sections that enable different learned models in {\name}. Let $\mathcal{B}$ be the cost budget. Costs in {\name} can be summarized as:  $$c_{\tt gen}  + c_{\tt pick} + c_{\tt gt} + c_{\tt AE} + c_{\tt GAN} + c_{\tt Model}\le\mathcal{B}.$$ In specific, $c_{\tt gen}$ and $c_{\tt pick}$ are both small in practice and can be done within a second.  $c_{\tt Model}$ is a constant overhead no matter if {\name} kicks in. $ c_{\tt AE}$ is a constant overhead that depends on the model sizes and data size in auto-encoder training. Moreover, $c_{\tt GAN}$ is also a constant overhead that depends on the number of iterations $n_{\tt g}$, model sizes and the number of queries generated in GAN training. Therefore, we consider the following as a proxy to the cost budget: $$c_{\tt gt}+C\le\mathcal{B}.$$ 
The constant factor $C$ can be measured by a simple runtime profiling or by counting the CPU cycles involved. We note that $s_{\tt gt}=n_{\tt gen}\cdot c_l$ is linear to the number of queries that need to be labeled. 
To this end, a key question here is that how many queries $n_{\tt gen}'$ should the generator produce and how many $n_{\tt train}$, $n_{\tt test}$, $n_{\tt gen}$ should the picker use for updating $\mathbb{M}$. We note the following cases and describe the solutions in {\name}. 

\vspace{0.05in}
\noindent\emph{Data shift.} Generating new queries is unnecessary in a data shift so that $n_{\tt gen}=0$. We assume no workload shift and {\name} uses $n_{\tt test}=0$ and $n_{\tt train}=s_{\tt gt}$ that fits the labeling budget. The picker $\mathbb{P}$ selects $n_{\tt train}$ queries from $\mathbb{I}_{\tt train}$.

\vspace{0.05in}
\noindent\emph{Workload shift.} Recall from Section~\ref{sec:method}, for {\tt case1} in which the test queries are adequate, $n_{\tt train}=n_{\tt gen}=0$ and training $\mathbb{M}$ uses whatever is available from the test workload $n_{\tt test}=s_{\tt query}$. For {\tt case2} when more queries need to be generated, the rule of thumb here is having similar query counts from the test and generated workloads $n_{\tt test}=n_{\tt gen}$, given that these two workloads are close enough. The picker $\mathbb{P}$ selects $n_{\tt gen}$ queries from the generated workload of the size $n_{\tt gen}'>n_{\tt gen}$. We will show in experiments this composition yields a promising model in general. We also note that the picker depends on the cost budget. \textcolor{red}{When $s_{\tt gt}$ or $\mathcal{B}$ is low}, more from the test workload has to be used and $n_{\tt test}>n_{\tt gen}$; in such a case we will show in ablation study that results are still reasonably good. That said, {\name} is insensitive to the composition among $n_{\tt train}, n_{\tt test}$ and $n_{\tt gen}$. 
Finally, for {\tt case3} when there are adequate test queries but the labeling cannot keep up, the configuration used here assembles that of the data shift case so that $n_{\tt test}=n_{\tt gen}=0$ and $n_{\tt train}=s_{\tt gt}$. 


\subsection{Triggers}
\noindent\textbf{Estimating $t$} can be done offline prior to {\name} kicks in  based on $\mathbb{M}$ and its original training corpus. As demonstrated in Figure \ref{fig:num}, $t$ is set to be the training size when the accuracy stabilizes. Doing so yields a robust \emph{initial} guess of $t$ which training and test workload match with each other. When there is a drift, beyond the initial guess made offline, we update $t$ on-the-fly when the {\name} kicks in. After each iteration in Algrirthm~\ref{alg:qgan}, we measure the gap $\delta$ between training and testing and adjust $t$ accordingly. Specifically, once $\delta>\theta_\delta$, indicating the test workload is more difficult than the training workload, we use $2\times$ of the initial $t$ guess. Meanwhile we pick $0.5\times$ of the $t$ guess when $\delta<0$. In our experiments we find this simple solution already yields good cutoff thresholds. 

\vspace{0.05in}
\noindent\textbf{Detecting data shift} can be achieved by counting the number of rows touched in-between training and testing. As suggested by [], re-training happens only when a significant portion of data has changed; {\name} inherits the practice here. 

\vspace{0.05in}
\noindent\textbf{Detecting workload shift} is achieved in {\name} using $\delta_0$, the accuracy gap of the CE model after the first iteration in Algorithm~\ref{alg:qgan}. Such metric is used as the switcher to kick in {\name}. Recall from Section ?, we consider this solution appropriate since it directly measures the accuracy degrade. 


\vspace{0.05in}
\noindent\textbf{Early stop in {\name}}. We measure $\delta$ after each iteration and use a threshold on $\delta$ as the early stopping criteria; this ensures that the gap due to shifts has been closed. 

\subsection{Implementation Details}
We implement a demonstration system of {\name} in Python. The CE models are black boxes as mentioned earlier while other learned modules  in {\name} including $\mathbb{G}, \mathbb{D}$ and $\mathbb{E}$ are implemented with PyTorch and sklearn. The query pool is a simple in-memory array and in our experiments, all input workloads from $\mathbb{I}_{\tt train}$ and $\mathbb{I}_{\tt test}$ have been cached in memory. The annotator $\mathbb{A}$ is a piece of C++ code. Our experiments are performed with Intel E5-2690 CPU; no GPU is used in our experiments, since most data centers are not equipped with GPUs. 


The learned modules in {\name} are implemented in different parallel processes due to the thread lock limitation in Python.  We defer to future work for refactoring {\name} in C++ so as to break this limit and improve efficiency. Nevertheless, our experiments already show improvements. Each module in {\name} pulls data from the pool and, when done with processing, pushes the outputs back to the pool.
To train the learned components in {\name}, a learning rate of 1e-3 is used with half-decay after every 10 epochs. Early stop is applied as described in Section ?. The auto-encoder task in qGAN is  pre-trained offline with queries used in training the original $\mathbb{M}$ and in such a manner the initial weights of $\mathbb{E}$ and $\mathbb{G}$ are determined; note that at this moment there is no test workload available. Lastly, when updating $\mathbb{M}$, we use a 5-fold cross-validation on the test workload and pick a better one due to the fact that updating $\mathbb{M}$ in general is inexpensive. 

%While training the M, we perform bootstrap training with two different methods: 1. with augmented workloads from qGAN; and 2. without augmented workloads. The system will reserve 20\% real workloads as a validation set, and then use the rest for bootstrap training. The system will choose the better tuned M model for weight update by evaluating on the validation set. This bootstrapping step could ensure M adapts accordingly even if qGAN fake workloads are not helpful for the real distribution. 

%\subsection{Discussions and Limitations}

\cut{
\subsection{Discussions and Limitations}

Runtime is slow, and the training time could be heavy for GAN

It could not help workload-agnostic models (e.g., DeepDB) because the qGAN system learns the workload distribution.

Estimation of t is not optimal, which could affect the qGAN system’s planning

The convergence of M could affect the efficiency of qGAN

If the M converges too fast on some simple dataset, the qGAN would not help too much

The convergence of qGAN could also affect the efficiency of adaptation

If the workload distribution is over complex, qGAN might take too long to converge.

In this case, the adaptation efficiency would be the same as the fine-tune baseline, but the CPU cycles on training the qGAN would be wasted



Interpretability: Similar to other NN-based methods, the interpretability of the qGAN is low.}

